UniK-QA: Unified Representations of Structured and Unstructured Knowledge for Open-Domain Question Answering

We study open-domain question answering with structured, unstructured and semi-structured knowledge sources, including text, tables, lists and knowledge bases. Departing from prior work, we propose a unifying approach that homogenizes all sources by reducing them to text and applies the retriever-reader model which has so far been limited to text sources only. Our approach greatly improves the results on knowledge-base QA tasks by 11 points, compared to latest graph-based methods. More importantly, we demonstrate that our unified knowledge (UniK-QA) model is a simple and yet effective way to combine heterogeneous sources of knowledge, advancing the state-of-the-art results on two popular question answering benchmarks, NaturalQuestions and WebQuestions, by 3.5 and 2.6 points, respectively. The code of UniK-QA is available at: https://github.com/facebookresearch/UniK-QA.

==> sections/analysis.tex <==
\section{Analysis}

\subsection{Retriever ablations}
\subsubsection{KBQA}
Comparing entity-linking + DPR vs. using DPR directly.
\begin{table}
\begin{center}
\begin{tabular}{|l|cc|}
\hline \bf Retrieval recall & \bf top-10 & \bf top-100 \\ \hline
All Wikidata &  &  \\
All NQ entitites, combined 2-hop & 1100 & 67.5 \\
\hline
Entity-linking + DPR & & \\
Direct DPR & & \\
\hline
\end{tabular}
\end{center}
\caption{\label{kbqa-retrieval-recall} Recall of answers in top-10 and top-100 passages for KB-only retriever on WebQ. }
\end{table}

Compare fixed quota vs. joint index for KB+text fusion.
\begin{table}
\begin{center}
\begin{tabular}{|l|cc|}
\hline \bf Retrieval recall & \bf WebQ & \bf NQ \\ \hline
Fixed quota & & \\
Joint index & & \\
\hline
\end{tabular}
\end{center}
\caption{\label{kbqa-retrieval-recall} Retrieval recall at top-100 passages. }
\end{table}

\subsubsection{Tables}
\begin{itemize}
    \item Compare fixed quota vs. joint index for tables+text fusion.
    \item Show iterative training is important to get joint index performing well.
    \item evaluate the impact of adding the table header heuristic
\end{itemize}

\begin{table}
\begin{center}
\begin{tabular}{|l|cc|}
\hline \bf Retrieval recall & \bf WebQ & \bf NQ \\ \hline
Fixed quota & & \\
Joint index & & \\
\hline
\end{tabular}
\end{center}
\caption{\label{kbqa-retrieval-recall} Retrieval recall at top-100 passages. }
\end{table}

